BLEU Meets COMET: Combining Lexical and Neural Metrics Towards Robust Machine Translation Evaluation

Although neural-based machine translation evaluation metrics, such as COMET or BLEURT, have achieved strong correlations with human judgements, they are sometimes unreliable in detecting certain phenomena that can be considered as critical errors, such as deviations in entities and numbers. In contrast, traditional evaluation metrics, such as BLEU or chrF, which measure lexical or character overlap between translation hypotheses and human references, have lower correlations with human judgements but are sensitive to such deviations. In this paper, we investigate several ways of combining the two approaches in order to increase robustness of state-of-the-art evaluation methods to translations with critical errors. We show that by using additional information during training, such as sentence-level features and word-level tags, the trained metrics improve their capability to penalize translations with specific troublesome phenomena, which leads to gains in correlation with human judgments and on recent challenge sets on several language pairs.

==> table1.tex <==
\begin{table}[ht]
\small
\centering
\addtolength{\tabcolsep}{-0.5pt}
% \resizebox{7.7cm}{!}{
\begin{tabular}{lccc}
\toprule
& r $\uparrow$ & $\rho$  $\uparrow$ & $\tau$ $\uparrow$ \\  
\midrule
BLEU  & 0.185 & 0.202 & 0.150 \\
chrF  & 0.210 & 0.236 & 0.176 \\
\textsc{Comet}  & 0.393 & 0.427 & 0.321 \\
% ensemble\_norm &  &  &  \\
ensemble  & 0.392 & 0.423 & 0.317 \\[0.1cm]
\bottomrule
\end{tabular}
\addtolength{\tabcolsep}{-0.5pt}
\caption{Average Pearson (r), Spearman ($\rho$) and Kendall's tau ($\tau$) correlations on a test set (MQM 2022). Weights for a weighted normalized ensemble are optimized on a development set (MQM 2021). For more detailed results per language pair see Tables~\ref{tab:mqm_kendall}, ~\ref{tab:mqm_pearson}, ~\ref{tab:mqm_spearman}.}
\label{tab:combined}
\end{table}

